Brane Physics in Non-Critical Theories

In this Thesis, we focus on the study of the low energy approximation to non-critical string theories. We present an exhaustive study of their solutions, which are divided in three cases: vacuum, NSNS charged, and RR charged solutions. In the first case, we find all possible solutions, including the previously known ones, which are special cases of ours. In the second case, we present the fundamental non-critical string, doubly localized in Minkowski \times the cigar vacuum. There are only a few known solutions doubly localized. Also, we completely solve the problem of finding NSNS solutions that fill all the Minkowski space. In the third case, we present new parametric families that contain some of the previously known solutions at particular values of the parameters. For the latter families, we have obtained the gauge duals in the context of the gauge/gravity duality, and we show that, in a particular region of the parameter space, these theories can confine. Finally, we study the obtained YM in D=3 and YM in D=4 theories, and we show the corresponding glueball spectra, that are in very good agreement with those predicted by lattice QCD.

==> append.tex <==
% Este cap\ii tulo colecciona los apendice.

\chapter{Apendices}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\appendix

\section{Some useful formulae I.}
\cleqn

Here we collect properties related with the ans\"atz for the fields assumed in
Section $2.1$,
\bea
G &=& -A^2\; dx^0{}^2+\tilde{A}^2\;d{\vec x}{}^2 + C^2\;d\rho^2 +
\tilde C^2\;dz^2\equiv\eta_{mn}\;\omega^m\;\omega^n\cr
A_{p+1} &=& dx^0\wedge\dots\wedge dx^p\; E(\rho)\cr
\Phi &=& \Phi(\rho)\label{ansatzapen}
\eea
where $\vec x$ is a $p$ dimensional vector, and we have introduced the vielbein $\omega^n$ and
dual vector fields $e_m$, $e_m(\omega^n)=\delta_m^n$, defined by,
\bea
\begin{array}{rclcrcl}
\omega^0&=&A(\rho)\;dx^0
\;\;\;\;&,&\;\;\;\; e_0 &=& A(\rho)^{-1}\;\partial_0\cr
\omega^{I}&=&\tilde A(\rho)\;dx^I
\;\;\;\;&,&\;\;\;\; e_I &=& \tilde A (\rho)^{-1}\;\partial_I\qquad,\qquad I=1,\dots,p\cr
\omega^{p+1}&=&C(\rho)\;d\rho
\;\;\;\;&,&\;\;\;\; e_{p+1}&=& C(\rho)^{-1}\;\partial_{\rho}\cr
\omega^{p+2}&=&\tilde C(\rho)\; dz
\;\;\;\;&,&\;\;\;\; e_{p+2} &=& \tilde C(\rho)^{-1}\;\partial_z
\end{array}
\eea
\subsection{Connections.}

As usual, the connections $\omega^m{}_n$ are completely determined by
\begin{itemize}
\item  No torsion condition: \hspace{2cm}$d\omega^m+{\omega^m}_n\wedge \omega^n=0$
\item  Metricity:\hspace{4cm}$\omega_{mn}\equiv\eta_{mp}\,\omega^p{}_n =-\omega_{nm}.$
\end{itemize}
From the direct computation of the coefficients ${\;\alpha^m}_{nl}$,
\begin{equation}
d\omega^m \equiv {1\over2}{\alpha^m}_{n l}\;\omega^n \wedge
\omega^l\;\;\;,\;\;\; {\alpha^m}_{nl} = - {\alpha^m}_{ln}
\end{equation}
we get the connections in the form,
\be
\omega_{mn}\equiv\omega_{m n l}\;\omega^l\qquad,\qquad
\omega_{m n l}={1\over2}(\alpha_{mn l}-\alpha_{l m n}+\alpha_{n l m})
\ee
We resume the non zero connections associated with the metric in (\ref{ansatzapen}),
\begin{eqnarray}
\omega_{0 p+1}&=&{\partial_{\rho}\ln A\over C}\;\omega_0= e_{p+1}(\ln A)\;\omega_0 \cr
\omega_{I p+1}&=&{\partial_{\rho}\ln \tilde A\over C}\;\omega_I
=e_{p+1}(\ln\tilde A)\;\omega_I\cr
\omega_{p+1,p+2}&=&-{\partial_{\rho}\ln\tilde C\over C}\;\omega_{p+2}=
-e_{p+1}(\ln \tilde C)\;\omega_{p+2}\label{conexiones}
\end{eqnarray}

\subsection{Covariant derivatives.}

We collect here covariant derivatives of interest related to the connections presented before.
By definition,
\begin{center}
$D_m(A_n)\equiv e_m(A_n)-\omega_{s n m}\; A_s$
\end{center}
Because in our equations we have scalar functions of $\rho$, it is enough to know a few of them.
Let $\phi(\rho)$ be an arbitrary scalar function; then we have the following
non zero derivatives (contraction of indices is assumed),
\begin{eqnarray}
D_{p+1}(\phi) &=& e_{p+1}(\phi) = \frac{1}{C}\,\partial_{\rho}\phi\cr
D_0{}^2(\phi)&=&-\frac{1}{C^2}\;\partial_{\rho}\ln A\;\partial_{\rho}\phi\cr
D_I D_J (\phi)&=&\delta_{IJ}\;e_{p+1}(\ln\tilde A)\;e_{p+1}(\phi)\cr
D_{p+1}{}^2(\phi)&=&\partial_{\rho}\left({\partial_{\rho}\phi\over C^2}\right)
+ \frac{1}{C^2}\;\partial_{\rho}\ln C\;\partial_{\rho}\phi\cr
D_{p+2}{}^2(\phi)&=& \frac{1}{C^2}\;\partial_{\rho}\ln \tilde C \;\partial_{\rho}\phi\cr
D^2(\phi) &=& \frac{1}{F_1}\;\partial_{\rho}\left(\frac{F_1}{C^2}\;\partial_{\rho}\phi\right)
=\partial_{\rho}\left(\frac{\partial_{\rho}\phi}{C^2}\right)+
\frac{1}{C^2}\;\partial_{\rho}\ln F_1\;\partial_{\rho}\phi\cr
e^{b\xi}D(e^{-b\xi}\; \psi\; D(\phi)) &=&\frac{1}{F_1\, e^{-b\xi}}\;\partial_{\rho}\left(\frac{F_1\,e^{-b\xi}}{C^2}\;
\psi\;\partial_{\rho}\phi\right)\cr
& & \label{derivadascov}
\end{eqnarray}
where $F_1 \equiv A\,\tilde A^p\, C\,\tilde C\;$,
$\;\epsilon_G =  dx^0\wedge dx^1\wedge\dots\wedge dx^p\wedge d\rho\wedge
d\theta \;F_1\,$.


\subsection{Curvature tensor.}

By definition,
\be
\Re_{mn} \equiv d\omega_{mn} + \omega_{mp}\wedge\omega^p{}_n =
\frac{1}{2}\,\Re_{mnpq}\;\omega^p\wedge\omega^q
\ee
The computation yields,
\bea
\Re_{0I}&=& D_0{}^2(\ln \tilde A)\;\omega_0\wedge\omega_I\cr
\Re_{0p+1}&=&-{1\over{A}}{D_{p+1}}^2(A)\;\omega_0\wedge\omega_{p+1}\cr
\Re_{Ip+1}&=&-{1\over{\tilde{A}}}D_{p+1}{}^2(\tilde{A})\;\omega_I\wedge\omega_{p+1}\cr
\Re_{IJ}&=&- D_{p+1}(\ln\tilde A)^2\;\omega_I\wedge\omega_J\cr
\Re_{0p+2}&=&-\frac{1}{A}D_{p+2}{}^2(A)\;\omega_0\wedge\omega_{p+2}\cr
\Re_{Ip+2}&=&-\frac{1}{\tilde A}D_{p+2}{}^2(\tilde{A})\;\omega_I\wedge\omega_{p+2}\cr
\Re_{p+1p+2}&=&-{1\over{\tilde{C}}}D_{p+1}{}^2(\tilde C)\;\omega_{p+1}\wedge\omega_{p+2}
\label{curvatura}
\eea


\subsection{Ricci tensor and Ricci scalar.}

From (\ref{curvatura}), we get the following components of the Ricci tensor
$R_{mn} \equiv \Re^p{}_{mpn}$,
%\vfill\eject
\bea
R_{00}&=& D^2(\ln A)\cr
R_{IJ}&=&- D^2(\ln \tilde A)\;\delta_{IJ}\cr
R_{p+1p+1}&=&-D^2(\ln C)-{1\over A}\partial_{\rho}\left({\partial_{\rho}A\over
C^2}\right)-{p\over \tilde A}\partial_{\rho}
\left({\partial_{\rho}\tilde A\over C^2}\right)+
{1\over C}\partial_{\rho}\left({\partial_{\tilde
\rho}C\over C^2}\right)- {1\over \tilde C}\partial_{\rho}
\left({\partial_{\rho}\tilde C\over C^2}\right)\cr
&=&-D^2(\ln C) - \frac{D_{p+1}{}^2(A)}{A} - p\,\frac{D_{p+1}{}^2(\tilde A)}{\tilde A}
+\frac{D_{p+1}{}^2(C)}{C} -\frac{D_{p+1}{}^2(\tilde C)}{\tilde C}\cr
&+&\frac{1}{C^2}\;\partial_{\rho}\ln C\;\partial_{\rho}\ln \frac{F_1}{C^2}\cr
R_{p+2p+2}&=&- D^2(\ln \tilde C)
\label{ricci}
\eea
\bigskip
The curvature scalar results,
\bea
R&=&
-{2\over C}\partial_{\rho}^2\left({1\over C}\right)
-D(\ln A)^2-p\,D(\ln \tilde A)^2-D(\ln C)^2-D(\ln \tilde C)^2\cr
&-&2\,D^2(\ln F_1)+D(\ln F_1)^2
\eea
\label{ricciscalar}

\subsection{Strength field tensor.}

With the ans\"atz in (\ref{fieldansatz}) for the $p+1$ form we get,
\begin{eqnarray}
F_{p+2} &=& dx^0\wedge\dots\wedge dx^p\; \partial_\rho E(\rho)\cr
\left(F_{p+2}\right)^2_{\mu\nu}&=&-{(\partial_{\rho}E)^2\over(A\,\tilde{A}^p\,C)^2}\;
\eta_{\mu \nu}\cr
\left(F_{p+2}\right)^2_{p+1p+1}&=&-
{(\partial_{\rho}E)^2\over(A\,\tilde{A}^p\,C)^2}\;
\end{eqnarray}

The gauge contribution to the strength field tensor results,

\begin{eqnarray}
T^A_{\mu\nu}&=&-\frac{2-b_p}{8}\;\frac{e^{(2+ b_p)\Phi}}{\left(A\,{\tilde A}^p\,C\right)^2}\;
\; (\partial_{\rho}E)^2\;\eta_{\mu\nu}\cr
T^A_{p+1p+1}&=&-\frac{2-b_p}{8}\;\frac{e^{(2+ b_p)\Phi}}{\left(A\,{\tilde A}^p\,C\right)^2}\;
\; (\partial_{\rho}E)^2\cr
T^A_{p+2p+2}&=&\frac{2+b_p}{8}\;\frac{e^{(2+ b_p)\Phi}}{\left(A\,{\tilde A}^p\,C\right)^2}\;
\; (\partial_{\rho}E)^2\label{fieldstrength}
\end{eqnarray}

\subsection{The equations of motion.}

With the help of the precedent results for the Ricci tensor, strength
field tensor, etc., the equations of motion (\ref{ecformal}) for the
ans\"atz (\ref{fieldansatz}) can be recast in the following way,
\bigskip

%%%% A-equation
\noindent\underline{$A$-equation}
\be
e^{2\Phi}D(e^{-2\Phi}D(\ln A))={2-b_p\over 8}\;{e^{(b_p+2)\Phi}\over (A{\tilde A}^p\,C)^2}\;
(\partial_\rho E)^2\label{1}
\ee
%%%%% \tilde A-equation
\noindent\underline{$\tilde A$-equation}
\be
e^{2\Phi}D(e^{-2\Phi}D(\ln \tilde A))=
{2-b_p\over 8}\;{e^{(b_p+2)\Phi}\over(A{\tilde A}^p\,C)^2}\;(\partial_\rho E)^2\label{2}
\ee
%%%% C-equation
\noindent\underline{$C$-equation}
\bea
&-&e^{2\Phi}D(e^{-2\Phi}D(\ln C))={D_{p+1}{}^2(A)\over A} + p\,{D_{p+1}{}^2(\tilde A)\over
\tilde A}- {D_{p+1}{}^2(C)\over C} + {D_{p+1}{}^2(\tilde C)\over \tilde C}\cr
&-&2\,D_{p+1}{}^2(\Phi)
-\frac{1}{C^2}\; \partial_\rho\ln C\;\partial_\rho\ln\left({F_1\over C^2}e^{-2\Phi}\right)
- \frac{2-b_p}{8}\;{e^{(b_p+2)\Phi}\over (A{\tilde A}^p\,C)^2}\;(\partial_\rho E)^2\label{3}
\eea
%%%%%%%% \tilde C-equation
\noindent\underline{$\tilde C$-equation}
\be
-e^{2\Phi}D(e^{-2\Phi}D(\ln \tilde C))={2+b_p\over 8}\;
{e^{(b_p+2)\Phi}\over (A{\tilde A}^p\,C)^2}\;(\partial_\rho E)^2\label{4}
\ee
%%%%%%%% Phi-equation
\noindent\underline{$\Phi$-equation}
\be
e^{2\Phi}D(e^{-2\Phi}D(\ln e^{-2\Phi}))=\Lambda^2 - (p+1)\,{2-b_p\over 8}\;
{e^{(b_p+2)\Phi}\over (A\tilde A^p\,C)^2}\;(\partial_\rho E)^2\label{5}
\ee
%%%% E-equation
\noindent\underline{E-equation}
\be
-D\left(\frac{e^{b_p\Phi}}{(A{\tilde A}^p)^2}\;D(E)\right)=
(-)^p \,Q_p\;\frac{\delta^2_{\perp}}{F_1}\label{6}
\ee
In the last one, the $E$-equation, we used the relation,
\be
*F_{p+2} = (-)^p\;\frac{\tilde C^2}{F_1}\;\partial_{\rho}E\;dz
\ee
and assumed a source of the form $\,Q_p\,J_{p+1}$,
\be
J_{p+1}^{01\dots p} = \frac{\delta^2_\perp}{\sqrt{-\det G}}=
\frac{\delta^2_{G^\perp}}{A\,\tilde A^p}\;\;\longrightarrow\;\;
J_{p+1} = -\delta^2_{G^\perp}\;\omega^0\wedge\dots\wedge\omega^p
\ee
where $G^\perp$ stands for the metric of the space where the flat $p$ brane is localized.



%\appendix


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% APPENDIX A %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Some useful formulae II.}\label{AA}


In this appendix we resume the conventions and formulae relevant in the computations carried out in the paper,
Unless specified on the contrary, we work in a local basis with indices $A, B, C,\dots=0,1,\dots,D-1$.

Let us consider a metric of the form,
\be
G = \eta_{AB}\;\omega^A\,\omega^B = \eta_{ab}\;\omega^a\,\omega^b + \omega^n{}^2\qquad,\qquad a,b = 0,1,\dots,D-2
\label{metrica}
\ee
where the vielbein $\omega^A$, dual vector fields $e_A ,\, e_A(\omega^B) = \delta_A^B\,$, and volume element are,
\bea
\omega^a &=& A_a(u)\,dx^a\qquad,\qquad e_a= A_a(u)^{-1}\,\partial_a\cr
\omega^n &=& C(u)\,du \qquad\;\;\;,\qquad e_n= C(u)^{-1}\,\partial_u\cr
\epsilon_G&=& \omega^0\wedge\dots\wedge\omega^n = dx^0\wedge\dots\wedge dx^{D-2}\wedge du\, F_1
\qquad,\qquad F_1 = \prod_a A_a\;C
\eea
The pseudo-riemmanian connections, $\,\omega_{AB}=-\omega_{BA}\,:\, d\omega^A+ \omega^A{}_B\wedge \omega^B=0\;$ are,
\bea
\omega_{ab} =
0\qquad &,&\qquad \omega_{an} = \sigma_a\,\omega_a\cr
\sigma_a\equiv e_n(\ln A_a)\qquad &,&\qquad \sigma\equiv
\sum_a\,\sigma_a = e_n\left(\ln\frac{F_1}{C}\right)\label{conn}
\eea
The relevant covariant derivatives on a scalar field $\phi(x,u)$ are,
\bea
D_A(\phi) &=& e_A(\phi)\qquad,\qquad \forall A\cr
D_a D_b(\phi)&=& e_a e_b(\phi) + \sigma_a\,e_n(\phi)\,\eta_{ab}\cr
D_a D_n(\phi)&=& e_a e_n(\phi) - \sigma_a\,e_a(\phi) \cr
D_n D_a(\phi)&=& e_n e_a(\phi) = D_a D_n(\phi)\cr
D_n{}^2 (\phi) &=& e_n{}^2 (\phi)\cr
D^2(\phi) &=& e^a e_a(\phi) + e_n{}^2(\phi) + \sigma\,e_n(\phi) = \sum_a \frac{\partial^a\partial_a\phi}{A_a{}^2}
+ \frac{1}{E}\,\partial_u\left(\frac{E}{C^2}\;\partial_u\phi\right)
%\cre^{b\xi}D^A\left(e^{-b\xi}\,\Psi\,D_A(\phi)\right) &=& e^{b\xi}D^a\left(e^{-b\xi}\,\Psi\,D_a(\phi)\right) +
%{e^{b\xi} \over F_1}\,\partial_u\left(\frac{F_1}{C^2}\,e^{-b\xi}\;\Psi\;\partial_u\phi\right)
\eea
with $\sigma$ defined in (\ref{conn}).

The relevant covariant derivatives on a one-form $A = A_A(x,u)\,\omega^A$ are,
\bea
D_b A_a&=& e_b (A_a) + \sigma_b\,A_n\,\eta_{ab}\cr
D_n A_a&=& e_n (A_a)\cr
D_a A_n&=& e_a (A_n) - \sigma_a\,A_a\cr
D_n A_n&=& e_n(A_n)\cr
D_c D_a A_b&=& e_c e_a (A_b) + \sigma_c\,e_n(A_b)\,\eta_{ca}-\sigma_c\,\sigma_a\, A_a\,\eta_{cb}
+ \sigma_b\,\left(e_c(A_n)\,\eta_{ab} + e_a(A_n)\,\eta_{cb}\right)\cr
D_n D_a A_b&=& e_n e_a (A_b) + e_n( \sigma_a\,A_n)\,\eta_{ab}\cr
D_a D_n A_b&=& e_a e_n (A_b) - \sigma_a\,e_a(A_b)
+ \sigma_b\,\left(e_n(A_n) - \sigma_b\,A_n\right)\,\eta_{ab}\cr
D_n D_n A_b &=& e_n{}^2(A_b)\cr
D_c D_a A_n&=& e_c e_a (A_n) - \sigma_a\,e_c(A_a)-\sigma_c\,e_a(A_c)
+ \sigma_a\,\left(e_n(A_n) - \sigma_a\,A_n\right)\,\eta_{ac}\cr
D_n D_a A_n&=& e_n e_a (A_n) - e_n( \sigma_a\,A_a)\cr
D_a D_n A_n&=& e_a e_n (A_n) - \sigma_a\,\left(e_a(A_n) + e_n(A_a) - \sigma_a\,A_a\right)\cr
D_n D_n A_n &=& e_n{}^2(A_n)
\eea
The relevant covariant derivatives on symmetric two-tensors $h=h_{AB}(x,u)\,\omega^A \,\omega^B$ are,
\bea
D_c h_{ab} &=& e_c(h_{ab}) + \sigma_c\,\left(\eta_{ac}\,h_{bn} + \eta_{bc}\,h_{an} \right)\cr
D_c h_{an} &=& e_c(h_{an}) + \sigma_c\,\left(\eta_{ac}\,h_{nn} - h_{ac}\right)\cr
D_c h_{nn} &=& e_c(h_{nn}) - 2\,\sigma_c\,h_{cn}\cr
D_n h_{AB} &=& e_n(h_{AB})\qquad,\qquad \forall\;\; A,B\cr
D_d D_c h_{ab} &=& e_de_c(h_{ab}) + \sigma_c\,\sigma_d\left( (\eta_{bc}\, \eta_{ad}+\eta_{ac}\, \eta_{bd})\, h_{nn}
- \eta_{ad}\,h_{bc}-\eta_{bd}\,h_{ac}\right)\cr
&+&\sigma_c\,\left( \eta_{cd}\, e_n(h_{ab}) + \eta_{ac}\, e_d(h_{bn}) + \eta_{bc}\, e_d(h_{an}\right)
+\sigma_d\,\left( \eta_{ad}\, e_c(h_{bn}) + \eta_{bd}\, e_c(h_{an})\right)\cr
D_n D_c h_{ab} &=& e_n e_c(h_{ab}) + \eta_{ac}\, e_n(\sigma_c\,h_{bn}) + \eta_{bc}\, e_n(\sigma_c\,h_{an})\cr
D_c D_n h_{ab} &=& e_c e_n(h_{ab}) + \sigma_c\left(\eta_{ac}\, e_n(h_{bn})+\eta_{bc}\, e_n(h_{an})-e_c(h_{ab})\right)
- \sigma_c{}^2\,\left(\eta_{ac}\, h_{bn} +\eta_{bc}\, h_{an}\right)\cr
D_d D_c h_{an} &=& e_d e_c(h_{an}) -\sigma_c\,\sigma_d\,\left(\eta_{ac}\, h_{dn} + 2\,\eta_{ad}\,h_{cn}\right)
+ \sigma_c\,\left(\eta_{ac}\, e_d(h_{nn}) - e_d(h_{ac})\right)\cr
&+& \sigma_d\,\left(\eta_{ad}\, e_c(h_{nn}) - e_c(h_{ad}\right)
+ \sigma_d\,\eta_{cd}\,\left(e_n(h_{an}) - \sigma_c\,h_{an}\right)\cr
D_n D_c h_{an} &=& e_n e_c(h_{an}) + \eta_{ac}\, e_n(\sigma_a\,h_{nn}) - e_n(\sigma_c\,h_{ac})\cr
D_c D_n h_{an} &=& e_c e_n(h_{an}) + \sigma_c\,\left(\eta_{ac}\, e_n(h_{nn})- e_n(h_{ac})-e_c(h_{an})\right)
- \sigma_c{}^2\,\left(\eta_{ac}\, h_{nn} - h_{ac}\right)\cr
D_d D_c h_{nn} &=& e_d e_c (h_{nn}) -2\,\sigma_c\, \sigma_d\,\left(\eta_{cd}\, h_{nn}- h_{cd}\right)
+ \sigma_c\,\eta_{cd}\, e_n(h_{nn})\cr
&-&2\,\left(\sigma_c\, e_d(h_{cn})+ \sigma_d\,e_c(h_{dn})\right)\cr
D_n D_c h_{nn} &=& e_n e_c(h_{nn}) -2\, e_n(\sigma_c\,h_{cn})\cr
D_c D_n h_{nn} &=& e_c e_n(h_{nn}) -\sigma_c\,\left(e_c(h_{nn})+ 2\,(e_n(h_{cn})-\sigma_c\,h_{cn})\right)\cr
D_n D_n h_{AB} &=& e_n{}^2(h_{AB})\qquad,\qquad \forall\;\; A,B\label{metricderiv}
\eea
The curvature tensor
$\,\Re_{AB} \equiv d\omega_{AB} + \omega_{AC}\wedge\omega^C{}_B \,$ is,
\bea
\Re_{ab}&=&-\sigma_a\,\sigma_b\;\omega_a\wedge\omega_b\cr
\Re_{an}&=&-\frac{1}{A_a}\, e_n{}^2(A_a)\;\omega_a\wedge\omega_n
\label{curvaturaII}
\eea
and the Ricci tensor and scalar are,
\bea
R_{ab}&=& -D^2(\ln A_a)\;\eta_{ab}\cr
R_{nn}&=&-\sum_a\,\frac{1}{A_a}\,
e_n{}^2(A_a)= - \left(e_n(\sigma) + \sum_a\sigma_a{}^2\right)\cr
R&=&  - 2\, D^2\left(\ln\frac{F_1}{C}\right) +\sigma^2 - \sum_a\sigma_a{}^2\label{riccis}
\eea

\subsection{Computation of the tensor $ A_{AB}$}\label{AA1}

The following symmetric two-tensor,
\be
A_{AB}(h) \equiv D_A D_B h^C_C + D^2 h_{AB} -  D^C D_A h_{CB} -D^C D_B h_{AC}
\ee
naturally arises in the metric perturbation theory.
With the help of (\ref{metricderiv}) we get the expressions,
\bea
A_{ab}(h) &=&  e^A e_A (h_{ab})+ e_a e_b(h^C_C)
-e_a e_n (h_{bn})-e_b e_n (h_{an}) -e^c e_a (h_{bc})-e^c e_b (h_{ac})\cr
&+&\sigma\,e_n(h_{ab}) +\left(  e_n(\sigma_a + \sigma_b) + \sigma\,(\sigma_a+\sigma_b) -
(\sigma_a-\sigma_b)^2 \right)\,h_{ab}\cr
&+& (2\,\sigma_a - \sigma_b -\sigma)\,e_a(h_{bn}) +
(2\,\sigma_b - \sigma_a -\sigma)\,e_b(h_{an})\cr
&+& \eta_{ab}\,\left(  -2\,\left( e_n(\sigma_a) + \sigma\,\sigma_a\right)\,h_{nn} +
\sigma_a\,\left( e_n(h^c_c) - e_n(h_{nn}) - 2\,\,e^c(h_{cn}\right) \right)\cr
A_{an}(h) &=& e^c e_c(h_{an}) - e^c e_n (h_{ac}) - e^c e_a (h_{cn}) + e_n e_a (h^c_c)
+2\, (e_n (\sigma_a) + \sigma\,\sigma_a )\, h_{an}\cr
&-& (\sigma - \sigma_a)\, e_a(h_{nn})+ (\sigma_a - \sigma_c)\, e^c(h_{ac}) + \sigma_c\,e_a(h^c_c)\cr
A_{nn}(h) &=& e^c e_c(h_{nn}) - \sigma\, e_n(h_{nn}) -2\, e^c e_n (h_{cn}) - 2\,\sigma_c\, e^c(h_{cn})
+ e_n{}^2 (h^c_c)+ 2\,\sigma_c\, e_n(h^c_c)\cr& &\label{AAB}
\eea
Under the gauge transformation in (\ref{gaugetrans}),
\bea
A_{ab}(\delta_\epsilon h) &=&
\left( e_n(\sigma_a) + \sigma\,\sigma_a + e_n(\sigma_b) + \sigma\,\sigma_b\right)\,
\delta_\epsilon h_{ab} + 2\, e_n\left( e_n(\sigma_a) + \sigma\,\sigma_a\right)\,\epsilon_n\,\eta_{ab}\cr
&+&\left( e_n(\sigma_b) + \sigma\,\sigma_b - e_n(\sigma_a) - \sigma\,\sigma_a \right)\,
\left(e_a(\epsilon_b) - e_b(\epsilon_a)\right)\cr
A_{an}(\delta_\epsilon h) &=&
2\,\left( e_n(\sigma_a) + \sigma\,\sigma_a\right)\,\delta_\epsilon h_{an} + 2
\left( \sum_c\left( e_n(\sigma_c) + \sigma_c{}^2\right) - e_n(\sigma_a) - \sigma\,\sigma_a\right)\,
e_a(\epsilon_n)\cr
A_{nn}(\delta_\epsilon h) &=& 2\, \sum_c\left( e_n(\sigma_c) + \sigma_c{}^2\right)\, \delta_\epsilon h_{nn}
+ 2\, e_n\left(\sum_c\left( e_n(\sigma_c) + \sigma_c{}^2\right)\right)\,\epsilon_n
\eea

\subsection{A short derivation of the solutions.}\label{AA2}

Here we sketch the obtention of the family of solutions (\ref{Ssn}) considered in the paper.
Let us consider an ans\"atz for the metric of the form (\ref{metrica}), together with,
\bea
\Phi(u) &=& \Phi = \rm{constant}\cr
F_D&=&(-)^D\,Q_{D-2}\;\epsilon_G\;\;\Longleftrightarrow\;\; *F_D= (-)^{D-1}\;Q_{D-2}\label{ansatz}
\eea
The strength field tensor in (\ref{ansatz}) leads to,
\bea
(F_D)^2{}_{AB} =
(F_D)^2\;\eta_{AB}\qquad,\qquad (F_D)^2 =-\left(\frac{C\;e_n(E)}{F_1}\right)^2
\eea
The equations of motion in string frame read (we consider D-branes, $b_{D-2}=0$),
\bea
R_{AB} &=&
\frac{1}{4}\, e^{2\Phi}\;\left(F_D\right)^2\;\eta_{AB}\cr
\Lambda^2 &=& - \frac{D}{4}\;e^{2\Phi}\; (F_D)^2\cr
d\left(*F_D\right)&=& (-)^D \; Q_{D-2}\; *J_{D-1}\;\;\;\;,\;\;\;\; Q_{D-2}\equiv 2\,\kappa_D{}^2\, \mu_{D-2} \label{ecformalII}
\eea
where $\kappa_D{}^2 =8\pi G_D$ is the gravitational coupling and $\mu_{D-2}$ the D$(D-2)$-brane tension.
The last two equations are solved by,
\be
\frac{C\; e_n(E)}{F_1}=-Q_{D-2}\qquad,\qquad e^{2\Phi} = \frac{4}{D}\;\frac{\Lambda^2}{Q_{D-2}{}^2}
\ee
while that the metric equations reduce to,
\bea
D^2(\ln A_a) \equiv e_n(\sigma_a) + \sigma\,\sigma_a &=&
\frac{\Lambda^2}{D}\,
%e^{\frac{4}{D-2}\Phi}
\qquad,\qquad \forall a\cr
\sum_a\,\left(e_n(\sigma_a) +
\sigma_a{}^2\right)&=&\frac{\Lambda^2}{D}\label{eqmetrica}
%e^{\frac{4}{D-2}\Phi}
\eea
By following steps similar to those in reference \cite{Lugo:2006vz}, the general solution to (\ref{eqmetrica})
can be written,
\be
A_a(u) = l_0\,u\,f(u)^\frac{a_a}{2}\qquad;\qquad C(u)=l_0\,u^{-1}\,f(u)^{-\frac{1}{2}}
\ee
with $f(u)$ as in (\ref{f}), and the constraints on the exponents given in (\ref{constraints}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% APPENDIX B %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The fluctuations in the T-dual solutions.}\label{AB}

\subsection{The family of solutions.}

The family of solutions (in string frame) obtained from .... by performing a T-duality transformation in,
i.e. $\,x^{D-2}-$ coordinate reads,
\bea
l_0{}^{-2}\,G &=& u^2\,f(u)^{a_\mu}\,\eta_{\mu\nu}\,dx^\mu\,dx^\nu + \frac{d u^2}{u^2\,f(u)}
+ u_1{}^2\,\frac{d\theta^2}{u^2\,f(u)^{a_\theta}}\qquad,\qquad \Lambda^2\,l_0{}^2 = D\,(D-1)\cr
e^{\Phi} &=& \frac{4\,\pi\,\sqrt{D-1}}{|Q_{D-3}|}\,\frac{u_1}{u}\,f(u)^{-\frac{a_\theta}{2}}\cr
F_{D-1} &=& \frac{Q_{D-3}\,l_0{}^{D-2}}{2\,\pi\,u_1}\,u^{D-2}\,du\wedge \,dx^0\wedge\dots\wedge dx^{D-3}
\;\;\leftrightarrow\;\; *F_{D-1} = (-)^{D-1}\,Q_{D-3}\,\frac{d\theta}{2\,\pi}\cr & &\label{sns}
\eea
where $\mu,\nu= 0,1,\dots,D-3\,$, the coordinate $\theta$ is $2\,\pi$-periodic, and the identifications
\be
f(u) = 1 - \left(\frac{u_0}{u}\right)^{D-1}
\ee
The scales $u_0$ and $u_1$ are arbitrary, and
Furthermore, the following constraints on the exponents must hold,
\be
\sum_\mu a_\mu+ a_\theta = 1\qquad,\quad \sum_\mu a_\mu{}^2 + a_\theta{}^2 = 1
\ee
Near horizon of D(D-3)-branes in a linear dilaton background...

Some useful relations are,
\bea
e_n(\sigma_\mu) + \sigma\,\sigma_\mu&=& \frac{\Lambda^2}{D-2}\,e^{\frac{4}{D-2}\,\Phi}\cr
e_n(\sigma_\theta) + \sigma\,\sigma_\theta &=& -\frac{D-4}{D (D-2)}\,\Lambda^2\,e^{\frac{4}{D-2}\,\Phi}\cr
\sum_a \left( e_n(\sigma_a) + \sigma_a{}^2\right)&=& \frac{\Lambda^2}{D-2}\,e^{\frac{4}{D-2}\,\Phi} -
\frac{4\,(D-2)}{(D-4)^2}\,\sigma_\theta{}^2\cr
\sigma^2 - \sum_a \sigma_a{}^2 &=& \frac{D-2}{D}\,\Lambda^2\,e^{\frac{4}{D-2}\,\Phi}
+ \frac{4\,(D-2)}{(D-4)^2}\,\sigma_\theta{}^2\cr
e_n{}^2(\Phi) + \sigma\,e_n(\Phi) &=& -\frac{\Lambda^2}{D}\,e^{\frac{4}{D-2}\,\Phi}\cr
e_n(\Phi)&=& \frac{D-2}{D-4}\,\sigma_\theta
\label{orig.rel}
\eea


\subsection{The  equations for the fluctuations in e-frame}

Being the system linear, it follows that $(L_\epsilon(G),L_\epsilon(\Phi),L_\epsilon(A_q))$ is solution for
any $\epsilon$, the pure gauge,
trivial, solution.
At difference of ordinary gauge or gravity theories, where the transformations are non linear, in this case it
should be possible to define explicitly gauge invariant quantities, and to express the equations for the
perturbations (\ref{ep1}) in terms of them in a manifest gauge invariant way.
In fact, for the family that will concern in this paper we can do it as follows.
First, we restrict ourselves to fluctuations such that,
\be
f_{D-1} \equiv \chi\, F_{D-1}\qquad,\qquad ^\epsilon\chi=\chi + D_{\tilde a}\epsilon^{\tilde a}
+ \frac{D}{D-4}\,\sigma_\theta\,\epsilon_n
\ee
Consistency with the Bianchi identity imposes $\theta$-independence of $\chi$, and therefore on all the
fluctuations; moreover the gauge transformation of $\chi$ follows from (\ref{gaugetrans}).
In second term, following (\ref{ls-bdgduals}) we introduce the fields $(g, g_a, I_{ab}, I_\xi,I_\chi)$ by,
\begin{eqnarray}
h_{nn} &\equiv& 2\,e_n(g) \qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad,\qquad\delta_\epsilon g = \epsilon_n\cr
h_{an} &\equiv& A_a\,e_n\left(\frac{g_a}{A_a}\right) + e_a(g)\;\;\qquad\qquad\qquad\qquad\qquad,\qquad\delta_\epsilon g_a = \epsilon_a\cr
h_{ab}&\equiv& I_{ab} + e_a(g_b) + e_b(g_a) + 2\,\eta_{ab}\,\sigma_a\, g\qquad\qquad\qquad,\qquad\delta_\epsilon I_{ab} = 0\cr
\xi &\equiv& I_\xi + \frac{D-2}{D-4}\,\sigma_\theta\, g\;\;\qquad\qquad\qquad\qquad\qquad\qquad,\qquad\delta_\epsilon I_\xi = 0\cr
\chi &\equiv& I_\chi + e^\mu(g_\mu) + e_n(g) + \left(\sigma + \frac{4}{D-4}\,\sigma_\theta\right)\,g
\qquad,\qquad\delta_\epsilon I_\chi = 0
\end{eqnarray}
where the gauge transformation follows from (\ref{gaugetrans}).
In terms of these variables (\ref{AAB}) is written as,
\bea
A_{ab}(h) &=& A^{(i)}_{ab}(I) + 2\, \left( e_n(\sigma_b) + \sigma\,\sigma_b\right)\,e_a(g_b)
+2\, \left( e_n(\sigma_a) + \sigma\,\sigma_a\right)\,e_b(g_a)\cr
&+& 2\,\eta_{ab}\,\left( e_n \left( e_n(\sigma_a) + \sigma\,\sigma_a\right)+
2\,\sigma_a\,\left( e_n(\sigma_a) + \sigma\,\sigma_a\right)\right) \,g\cr
A^{(i)}_{ab}(I)&\equiv& e^A e_A (I_{ab})+ e_a e_b(I^c_c)- e_ae^c (I_{bc})- e_be^c (I_{ac})+\sigma\,e_n(I_{ab})\cr
&+&\left(  e_n(\sigma_a + \sigma_b) + \sigma\,(\sigma_a+\sigma_b) -(\sigma_a-\sigma_b)^2 \right)\,I_{ab}
+ \eta_{ab}\,\sigma_a\, e_n\left(I^c_c\right)\cr
A_{an}(h) &=& A^{(i)}_{an}(I) + 2\, \left( e_n(\sigma_a) + \sigma\,\sigma_a\right)\,
\left( e_n(g_a) - \sigma_a\,g_a\right)+ 2\,\sum_c \left( e_n(\sigma_c) + \sigma_c{}^2\right)\; e_a(g)\cr
A^{(i)}_{an}(I)&\equiv&- e^c e_n (I_{ac}) + e_a e_n (I^c_c) + (\sigma_a - \sigma_c)\,
\left( e^c(I_{ac}) - \,e_a(I^c_c)\right)\cr
A_{nn}(h) &=&A^{(i)}_{nn}(I) +4\,\sum_c \left( e_n(\sigma_c) + \sigma_c{}^2\right)\; e_n(g) +
2\, e_n\left(\sum_c \left( e_n(\sigma_c) + \sigma_c{}^2\right)\right)\; g\cr
A^{(i)}_{nn}(I)&\equiv& e_n{}^2 (I^c_c)+ 2\,\sigma_c\, e_n(I^c_c)\label{Ainv}
\eea
By using these expressions, the equations (\ref{ep1}) in our backgrounds result,
\bea
0 &=& e^A e_A (I_{\mu\nu})+ e_\mu e_\nu(I^c_c)- e_\mu e^c (I_{\nu c})- e_\nu e^c (I_{\mu c})+\sigma\,e_n(I_{\mu\nu})\cr
&+&\eta_{\mu\nu}\,\sigma_\mu\, e_n\left(I^c_c\right)- \left(\sigma_\mu-\sigma_\nu \right)^2 \,I_{\mu\nu}
- \frac{8\,\Lambda^2}{(D-2)^2}\, \eta_{\mu\nu}\, e^{\frac{4}{D-2}\,\Phi}  \,I_\xi\cr
0 &=& - e^c e_n (I_{\mu c}) + e_\mu e_n (I^c_c) + (\sigma_\mu - \sigma_c)\,
\left( e^c(I_{\mu c}) - \,e_\mu (I^c_c)\right)+ \frac{8}{D-4}\, \sigma_\theta\, e_\mu (I_\xi) \cr
0 &=& e_n{}^2 (I^c_c)+ 2\,\sigma_c\, e_n(I^c_c)+ \frac{16}{D-4}\, \sigma_\theta\, e_n (I_\xi)
- \frac{8\,\Lambda^2}{(D-2)^2}\, e^{\frac{4}{D-2}\,\Phi} \,I_\xi \cr
0 &=& e^A e_A (I_{\theta\theta})+ \sigma\,e_n(I_{\theta\theta}) + \sigma_\theta\,e_n(I_c^c)
+ \frac{8\,\Lambda^2}{D}\, e^{\frac{4}{D-2}\,\Phi}\, \left( \,I_\chi -\frac{1}{2}\, I_\mu^\mu
- \frac{D^2 -3\,D +4}{(D-2)^2}\,I_\xi\right)\cr
0 &=& e^A e_A (I_{\mu\theta})+ \sigma\,e_n(I_{\mu\theta}) - e_\mu e^c(I_{c\theta})
+ \left( \frac{2\,\Lambda^2}{D}\, e^{\frac{4}{D-2}\,\Phi} - (\sigma_\mu -\sigma_\theta)^2\right)\,I_{\mu\theta}\cr
0 &=& e^c\left( e_n(I_{c\theta }) + (\sigma_c -\sigma_\theta)\,I_{c\theta}\right)\cr
0 &=& e^A e_A(I_\xi) + \sigma\, e_n(I_\xi)+ \frac{D-2}{2(D-4)}\,\sigma_\theta\,e_n(I_c^c)\cr
&+& \frac{D-2}{D}\,\Lambda^2\, e^{\frac{4}{D-2}\,\Phi}\, \left( -I_\chi +\frac{1}{2}\, I_\mu^\mu
+ \frac{D^2 -2\,D +4}{(D-2)^2}\,I_\xi\right)\cr
0&=& -e^{-\alpha_q\Phi}\,D^B\left(e^{\alpha_q\Phi}\,(f_{q+2})_{A_1\dots A_{q+1}B}\right)\qquad,\qquad q\neq D-3
\label{hxieqn}
\eea

\noindent\underline{ h-equations}

\bea
A_{\mu\nu}(h)\, e^{-\frac{4}{D-2}\,\Phi} &=& \frac{2\,\Lambda{}^2}{D-2}\, h_{\mu\nu} +
\frac{8\,\Lambda^2}{(D-2)^2}\,\eta_{\mu\nu}\,\xi\cr
A_{\mu n}(h)\, e^{-\frac{4}{D-2}\,\Phi} &=& \frac{2\,\Lambda{}^2}{D-2}\, h_{\mu n} -
\frac{8}{D-2}\,e^{-\frac{4}{D-2}\,\Phi}\,e_n(\Phi)\,e_\mu(\xi)\cr
A_{nn}(h)\, e^{-\frac{4}{D-2}\,\Phi} &=& \frac{2\,\Lambda{}^2}{D-2}\, h_{nn} -
\frac{16}{D-2}\,e^{-\frac{4}{D-2}\,\Phi}\,e_n(\Phi)\,e_n(\xi) + \frac{8\,\Lambda^2}{(D-2)^2}\,\xi\cr
A_{\theta\theta}(h)\, e^{-\frac{4}{D-2}\,\Phi} &=& -\frac{2\,(D-4)}{D (D-2)}\, \Lambda^2\,h_{\theta\theta} +
\frac{8 (D^2-3D+4)}{D(D-2)^2}\,\Lambda^2\,\xi +
\frac{4}{D}\,\Lambda^2\,\left( h^{\tilde a}_{\tilde a} - 2\,\chi\right)\cr
A_{\tilde a\theta}(h)\, e^{-\frac{4}{D-2}\,\Phi} &=& -\frac{2\,(D-4)}{D (D-2)}\,\Lambda{}^2\, h_{\tilde a\theta} -
\frac{8}{D-2}\, e^{-\frac{4}{D-2}\,\Phi}\, e_{\tilde a}(\Phi)\,e_\theta(\xi)\qquad,\qquad \tilde a\neq \theta\cr & &
\eea

\noindent\underline{$\xi$-equation}

\bea
e^{-\frac{4}{D-2}\,\Phi}\,D^2(\xi) &=& e^{-\frac{4}{D-2}\,\Phi}\,e_n(\Phi)\,
\left( e^A(h_{An}) - \frac{1}{2}\,e_n(h^A_A)\right)+ e^{-\frac{4}{D-2}\,\Phi}\,D^2(\Phi)\,h_{nn}\cr
&-& \frac{D-2}{2\,D}\,\Lambda^2\,h_{\theta\theta}  +\frac{D^2 -6\,D+4}{D (D-2)}\,\Lambda^2\,\xi
\eea

\noindent\underline{$a_{D-2}\,$-equation}
\bigskip

From the appendix we get a equation with $(D-2)$ antisymmetric indices that leads to the following equations,
\bea
0 &=&e_\mu (I_{\nu\theta}) -e_\nu (I_{\mu\theta})\qquad,\qquad \forall\, \mu,\nu\cr
0&=& e_n\left(\frac{A_\mu}{A_\theta}\,I_{\mu\theta}\right)\qquad,\qquad \forall\, \mu\cr
0&=& e_{\tilde a}\left(2\,I_\xi - I_\chi + \frac{1}{2}\,(I_\mu^\mu - I_{\theta\theta})\right)\qquad,\qquad \forall\,\tilde a
\eea
with solution,
\bea
I_{\mu\theta}&=&0\qquad,\qquad \forall\,\mu\cr
I_\chi &=& 2\,I_\xi  + \frac{1}{2}\,(I_\mu^\mu - I_{\theta\theta})
\eea
By introducing these values in (\ref{hxieqn}) we get the following system,
\bea
0 &=& e_n{}^2 (I_{\mu\nu})+ \sigma\,e_n(I_{\mu\nu}) + e^\rho e_\rho (I_{\mu\nu}) + e_\mu e_\nu(I^c_c)- e_\mu e^\rho (I_{\nu\rho})-
e_\nu e^\rho (I_{\mu\rho})- \left(\sigma_\mu-\sigma_\nu \right)^2 \,I_{\mu\nu}\cr
&+&\eta_{\mu\nu}\,\sigma_\mu\, e_n\left(I^c_c\right)- \frac{8\,\Lambda^2}{(D-2)^2}\, \eta_{\mu\nu}\, e^{\frac{4}{D-2}\,\Phi}\,I_\xi\cr
0 &=& e_n{}^2(I_{\theta\theta})+ \sigma\,e_n(I_{\theta\theta})+ e^\rho e_\rho (I_{\theta\theta})+ \sigma_\theta\,e_n(I_c^c)\cr
&+& \frac{8\,\Lambda^2}{D}\, e^{\frac{4}{D-2}\,\Phi}\, \left( \frac{(D-1)(D-4)}{(D-2)^2}\, I_\xi - \frac{1}{2}\,I_{\theta\theta}\right)\cr
0 &=& - e^\rho e_n (I_{\mu\rho}) + e_\mu e_n (I^c_c) + (\sigma_\mu - \sigma_\rho)\, e^\rho(I_{\mu\rho}) +
(\sigma_c - \sigma_\mu) \,e_\mu (I^c_c)+ \frac{8}{D-4}\, \sigma_\theta\, e_\mu (I_\xi) \cr
0 &=& e_n{}^2 (I^c_c)+ 2\,\sigma_c\, e_n(I^c_c)+ \frac{16}{D-4}\, \sigma_\theta\, e_n (I_\xi)
- \frac{8\,\Lambda^2}{(D-2)^2}\, e^{\frac{4}{D-2}\,\Phi} \,I_\xi \cr
0 &=& D^2(I_\xi) + \frac{D-2}{2(D-4)}\,\sigma_\theta\,e_n(I_c^c) - \frac{(D-2)\,\Lambda^2}{D}\, e^{\frac{4}{D-2}\,\Phi}\,
\left(\frac{D^2 -6D+4}{(D-2)^2}\, I_\xi - \frac{1}{2}\,I_{\theta\theta}\right)\cr& &\label{eqn1}
\eea
Now we introduce the modes in momenta,
\be
I_{\mu\nu} = \chi_{\mu\nu}(u)\,e^{i p\cdot x}\qquad;\qquad
I_{\theta\theta} = \chi_\theta(u)\,e^{i p\cdot x}\qquad;\qquad
I_\xi = \chi_\xi(u) \,e^{i p\cdot x}
\ee
where $p\cdot x \equiv p_\rho\,x^\rho\,$.
With the definition  $p_\mu \equiv A_\mu\,\tilde p_\mu\,$, we get the system in the form,
\bea
0 &=& e_n{}^2 (\chi_{\mu\nu})+ \sigma\,e_n(\chi_{\mu\nu}) - \left(\tilde p^\rho\, \tilde p_\rho +
\left(\sigma_\mu-\sigma_\nu \right)^2 \right)\,\chi_{\mu\nu} +
\tilde p_\mu \,\tilde p^\rho\,\chi_{\nu\rho}+\tilde p_\nu \,\tilde p^\rho\,\chi_{\mu\rho}\cr
&-&\tilde p_\mu\,\tilde p_\nu\, ( \chi^\rho_\rho + \chi_\theta)+
\eta_{\mu\nu}\,\sigma_\mu\, e_n\left(\chi^\rho_\rho + \chi_\theta\right)-
\frac{8\,\Lambda^2}{(D-2)^2}\, \eta_{\mu\nu}\, e^{\frac{4}{D-2}\,\Phi}\,\chi_\xi\cr
0 &=& e_n{}^2(\chi_\theta)+ \sigma\,e_n(\chi_\theta)-
\left( \tilde p^\rho \tilde p_\rho+\frac{4\,\Lambda^2}{D}\, e^{\frac{4}{D-2}\,\Phi}\right)\,\chi_\theta
+ \sigma_\theta\,e_n(\chi_\rho^\rho + \chi_\theta)\cr
&+& \frac{8(D-1)(D-4)}{D(D-2)^2}\,\Lambda^2\,e^{\frac{4}{D-2}\,\Phi}\, \chi_\xi \cr
0 &=& e_n{}^2(\chi_\xi)+ \sigma\,e_n(\chi_\xi) - \left( \tilde p{}^2+
\frac{D^2 -6D+4}{D(D-2)}\,\Lambda^2\, e^{\frac{4}{D-2}\,\Phi}\, \chi_\xi\right)
+ \frac{D-2}{2(D-4)}\,\sigma_\theta\,e_n(\chi^\rho_\rho + \chi_\theta)\cr
&+& \frac{D-2}{2\,D}\,\Lambda^2 e^{\frac{4}{D-2}\,\Phi} \,\chi_\theta\cr
0 &=& \tilde p^\mu\,\left( e_n (\chi^\rho_\rho + \chi_\theta) + (\sigma_\rho - \sigma_\mu) \,\chi^\rho_\rho
+ (\sigma_\theta - \sigma_\mu) \,\chi_\theta + \frac{8}{D-4}\, \sigma_\theta\,\chi_\xi\right) \cr
&-& \tilde p^\rho\,\left( e_n (\chi_{\mu\rho}) + (\sigma_\rho - \sigma_\mu)\,\chi_{\mu\rho} \right)\cr
0 &=& e_n{}^2 (\chi^\rho_\rho+\chi_\theta) + 2\,\sigma_\rho\, e_n(\chi^\rho_\rho)+
 + 2\,\sigma_\theta\, e_n(\chi_\theta)+\frac{16}{D-4}\, \sigma_\theta\, e_n (\chi_\xi)
- \frac{8\,\Lambda^2}{(D-2)^2}\, e^{\frac{4}{D-2}\,\Phi} \,\chi_\xi\cr & &
\label{eqn2}
\eea
We note that we have left with the unknowns $(\chi_{\mu\nu}, \chi_{\theta\theta}, \chi_\xi )$,
whose system of coupled, second order, differential equations is given by the first three equations;
the last two ones should work as constraints.


\subsection{Holographic models of $d$ dimensional Yang-Mills theories}


Let us take, among the $x^\mu $ coordinates, $d$ non compact, equivalent, $x^\alpha$-coordinates, $\alpha=0,1,\dots, d-1$,
and $D-d-2$ compact and non equivalent $\tau^i, i=1,\dots D-d-2, \tau_i\equiv \tau_i +2\,\pi\,R_i$.
We will denote with a $\tilde{} $ quantities associated with the non-compact directions
($A_\alpha = \tilde A\,,\, a_\alpha = \tilde a\, ,\,\sigma_\alpha = \tilde \sigma\,,\,$ etc).
The metric and constraints (\ref{constraints}) are,
\bea
l_0{}^{-2}\;G &=& u^2\left( f(u)^{\tilde a}\;\eta_{\mu\nu}\,dx^\mu\,dx^\nu + \sum_i\,f(u)^{a_i}\;d\tau^i{}^2\right)
+ \frac{du^2}{u^2\,f(u)}+ u_1{}^2\,\frac{d\theta^2}{u^2\,f(u)^{a_\theta}}\cr
& &d\,\tilde a + \sum_i a_i + a_\theta=1\qquad,\qquad d\,\tilde a^2 + \sum_i a_i{}^2+a_\theta{}^2 =1
\eea
We stress that $D-d-2$ exponents remain free.

\subsection{Metric:  transverse fluctuations}

They correspond to take the ans\" atz,
\be
\chi_{\alpha\beta}(u)= \epsilon_{\alpha\beta}(p)\;\chi(u)\qquad;\qquad
\epsilon_\alpha^\alpha=0\;\;,\;\;\epsilon_{\alpha\beta}\,p^\beta = 0\label{hmnanstransorig}
\ee
and the rest of the fluctuations zero.
This ans\" atz solves (\ref{eqn2}) if $\chi$ satisfies,
\be
e_n{}^2 (\chi)+ \sigma\,e_n(\chi) + \left( \frac{M^2}{\tilde A^2} - \sum_i \tilde p _i{}^2 \right)\,\chi=0
\ee
where $M^2\equiv -p^\alpha p_\alpha$ is the $d$-dimensional mass.
By making the change ..., it turns that H satisfy exactly the equation .....

\subsection{Metric: longitudinal fluctuations}

They correspond to take the ans\" atz, at fixed $i$ (but for any $i$),
\be
\chi_{i\alpha}(u)= \epsilon_\alpha(p)\;\chi(u)\qquad;\qquad
p_i=0\;\;,\;\;\epsilon_\alpha\,p^\alpha = 0\label{hmnanslongorig}
\ee
and the rest of the fluctuations zero.
It is consistent with (\ref{eqn2}) if $\chi(u)$ obeys,
\be
e_n{}^2 (\chi)+ \sigma\,e_n(\chi) + \left( \frac{M^2}{\tilde A^2} - \sum_i \tilde p _i{}^2
- (\tilde\sigma - \sigma_i{})^2\right)\,\chi=0
\ee
By making the change ..., it turns that H satisfy exactly the equation .....

\subsection{Scalar fluctuations}

We expect that they come from the dilaton and the metric.
However, at difference of the case worked out in references \cite{Constable:1999gb},
\cite{Kuperstein:2004yk}, they do not disentangle, in the sense that putting to zero
the metric fluctuations is not consistent.
So we start with the ans\" atz for the metric,
\be
\chi_{\mu\nu}(u) = a_\mu(u)\,\eta_{\mu\nu} + b_{\mu\nu}(u)\,p_\mu\,p_\nu
\ee
which at difference of the cases treated above, is not transverse neither traceless.
It results convenient to introduce the following variables,
\bea
\chi_\mu &\equiv& a_\mu - \sigma_\mu\, \frac{\chi_\theta}{\sigma_\theta}\cr
\tilde\chi_{\mu\nu} &\equiv& A_\mu\,A_\nu\, b_{\mu\nu} -
\frac{1}{2} ( A_\mu{}^2\, b_{\mu\mu} + A_\nu{}^2\, b_{\nu\nu})\cr
\tilde\chi_\mu &\equiv& A_\mu{}^2\, e_n(b_{\mu\mu}) - \frac{\chi_\theta}{\sigma_\theta}\cr
\tilde \chi_\theta &\equiv& e_n\left(\frac{\chi_\theta}{\sigma_\theta}\right)\cr
\tilde \chi_\xi&\equiv& \chi_\xi -\frac{D-2}{2(D-4)}\, \chi_\theta
\eea
We note that $b_{\mu\nu}$ is replaced by $\tilde\chi_{\mu\nu}$ and $\tilde\chi_\mu$ (by construction,
$\tilde\chi_{\mu\mu}\equiv 0$ for any $\mu$).
With them, and combining equations in (\ref{eqn2}), we can rearrange the system in the following way,
\bea
0 &=& e_n{}^2 (\chi_\mu)+ \sigma\,e_n(\chi_\mu) - \tilde p^\rho\, \tilde p_\rho\,\chi_\mu +
\frac{2\,\Lambda^2}{D-2}\, e^{\frac{4}{D-2}\,\Phi}\, \left( 1 +
\frac{D-4}{D}\,\frac{\sigma_\mu}{\sigma_\theta}\right)\,\tilde\chi_\theta\cr
&-&\frac{8\,\Lambda^2}{(D-2)^2}\, e^{\frac{4}{D-2}\,\Phi}\, \left( 1
+ (D-1)\frac{D-4}{D}\,\frac{\sigma_\mu}{\sigma_\theta}\right)\,\tilde\chi_\xi\cr
0 &=& e_n{}^2 (\tilde\chi_{\mu\nu})+ \left(\sigma -2(\sigma_\mu +\sigma_\nu)\right)\,e_n(\tilde\chi_{\mu\nu}) +
\sum_\rho \tilde p^\rho\, \tilde p_\rho \,\left( \tilde\chi_{\mu\rho}
+ \tilde\chi_{\nu\rho} - \tilde\chi_{\mu\nu}\right)\cr
&+& \left(  4\,\sigma_\mu \,\sigma_\nu  -\frac{2\,\Lambda^2}{D-2}\, e^{\frac{4}{D-2}\,\Phi}\right)\,\tilde\chi_{\mu\nu}
+ \tilde\chi_\theta + \chi_\mu + \chi_\nu-\sum_\rho\chi_\rho\cr
&+& \frac{1}{2}\,\left(e_n(\tilde\chi_\mu +\tilde\chi_\nu)
+\sigma\,(\tilde\chi_\mu +\tilde\chi_\nu)\right)-\sigma_\mu\,\tilde\chi_\nu -\sigma_\nu\,\tilde\chi_\mu\cr
0 &=& e_n{}^2(\tilde\chi_\xi)+ \sigma\,e_n(\tilde\chi_\xi) - \left( \tilde p{}^2
+ \Lambda^2\, e^{\frac{4}{D-2}\,\Phi}\right)\,\tilde\chi_\xi\cr
0 &=& \sigma_\theta\,e_n(\tilde\chi_\theta)+ 2\, D^2(\ln A_\theta)\,\tilde\chi_\theta
+ \sigma_\theta\,e_n(\sum_\rho\chi_\rho)
+ \sigma_\theta\, \sum_\rho \tilde p^\rho\,\tilde p_\rho\,\tilde\chi_\rho\cr
&+& \frac{8(D-1)(D-4)}{D(D-2)^2}\,\Lambda^2\,e^{\frac{4}{D-2}\,\Phi}\,\tilde\chi_\xi \cr
0 &=& \sum_\rho \left( e_n(\chi_\rho) + (\sigma_\rho - \sigma_\mu)\, \chi_\rho\right) - e_n(\chi_\mu)
+ (\sigma - \sigma_\mu)\, \tilde\chi_\theta +\frac{8}{D-4}\, \sigma_\theta\, \tilde\chi_\xi\cr
&-&\sum_\rho \tilde p^\rho\,\tilde p_\rho\,\left( \frac{1}{2}(\tilde\chi_\mu -\tilde\chi_\rho)
+ e_n(\tilde\chi_{\mu\rho}) - 2\,\sigma_\mu\,\tilde\chi_{\mu\rho}\right)\cr
0 &=& \sum_\rho \tilde p^\rho\,\tilde p_\rho\,
\left( \chi_\rho + (\sigma - \sigma_\rho)\, \tilde\chi_\rho
+\sum_\sigma\tilde p^\sigma\,\tilde p_\sigma\,\tilde\chi_{\rho\sigma}\right)
+\frac{D-2}{D}\,\Lambda^2\,e^{\frac{4}{D-2}\,\Phi}\,\left(\tilde\chi_\theta
- \frac{8}{(D-2)^2}\,\tilde\chi_\xi\right)\cr & &\label{eqn3}
\eea


==> appendIV.tex <==
\subsection*{La tensi\'on y la carga de la D-brana}

Para terminar, falta determinar $\tau_p$ y $\mu_p$ que aparecen en la
acci\'on de volumen de mundo de la D$p$-brana~\eqref{Dpwv}, a los
cuales hemos denominado la tensi\'on y la carga de R-R de la
D$p$-brana. Para poder determinarlas, es necesario calcular la amplitud
de vac\ii o de cuerdas entre D-branas~\cite{Polchinski:1995mt}.
Consideremos entonces dos D$p$-branas paralelas, localizadas
respectivamente en $x^i=0$ y en $x^i=y^i$. La energ\ii a libre a un
loop planar, para una cuerda abierta con $9-p$ condiciones de contorno
de Dirichlet est\'a dada por la f\'ormula de \emph{Coleman--Weinberg}:
\begin{equation}
	F = -2 \times \frac{1}{2}\tr \ln (L_0-a) = \int_0^{\infty}
        \frac{dt}{t}\tr_{\text{NS}-\text{R}}\left[\frac{1+(-1)^F}{2}e^{-2\pi
            t (L_0-a)}\right]\,,
\end{equation}
donde debemos tener en cuenta la proyecci\'on GSO y las dos posibles
orientaciones de la cuerda entre las dos branas:
\begin{equation}
	L_0 = \ls^2 p^2 + \frac{y^2}{(2\pi\ls)^2} +
        \sum_{n=1}^{\infty} \alpha_{-n} \cdot \alpha_n + \sum_{r>0} r
        \psi_{-r} \cdot \psi_r\,,
\end{equation}
donde ahora $p$ s\'olo denota el momento en las direcciones
longitudinales. El c\'alculo expl{\'\i}cito de la traza en los diferentes
sectores da como resultado:
\begin{equation}\label{polchinski}
	F = V_{p+1} \int_{0}^{\infty}
        \frac{dt}{2t}\ (8\pi^2\ls^2t)^{-\frac{p+1}{2}} e^{-\frac{y^2
            t}{2\pi\ls^2}}\ \frac{f_3(q)^8 - f_4(q)^8 -
          f_2(q)^8}{f_1(q)^8}\,,
\end{equation}
donde $V_{p+1}$ es el volumen de la brana (infinito), $q=e^{-2\pi t}$ y
\begin{equation}
\begin{aligned}
	f_1(q) &= q^{1/24}\prod_{n=1}^{\infty} ( 1 - q^n )\,,& f_2(q)
        &= \sqrt{2}q^{1/24}\prod_{n=1}^{\infty} ( 1 + q^n
        )\,,\\ f_3(q) &= q^{-1/48}\prod_{n=1}^{\infty} ( 1 + q^{n-1/2}
        )\,,& f_4(q) &= q^{-1/48}\prod_{n=1}^{\infty} ( 1 - q^{n-1/2}
        )\,.
\end{aligned}
\end{equation}

La amplitud~\eqref{polchinski} se anula debido a la ``abstruse
identity'' satisfecha por la funci\'on $f_i(q)$, y esto significa que
no hay fuerzas entre dos branas paralelas de igual dimensi\'on,
consecuencia de la supersimetr\ii a. Sin embargo, es posible extraer
informaci\'on de la tensi\'on de la cuerda, as{\'\i} como de su carga,
notando que la amplitud a un loop que hemos computado es justamente un
diagrama tipo anillo, que puede ser tratado como una amplitud de
cuerda cerrada a nivel \'arbol, con la topolog\ii a de un cilindro y
que puede ser interpretada como la emisi\'on y sucesiva absorci\'on de
una cuerda cerrada por una brana. Esto es realizado expl\ii citamente
e implementando la transformaci\'on modular $t\to s=1/t$ al canal de
cuerda cerrrada. La anulaci\'on de la amplitud~\eqref{polchinski} es
entonces interpretada como una cancelaci\'on mutua de las fuerzas
atractivas (de tipo gravitacional) debidas a los campos en el sector
de $NS-NS$ de las cuerdas cerradas con la fuerzas repulsivas (de tipo
electromagn\'etico) debido a los campos del sector de $R-R$:
\begin{equation}
	F = \mathcal{A}_{\text{NS-NS}}+\mathcal{A}_{\text{R-R}}=0\,.
\end{equation}
En el l\ii mite $s\to\infty$, la amplitud es dominada por los campos
de cuerdas cerradas livianas, las no masivas. Podemos entonces
desarrollar el resultado~\eqref{polchinski} (despu\'es de realizar una
transformaci\'on modular) obteniendo:
\begin{equation}\label{pole}
	\mathcal{A}_{\text{NS-NS}}=-\mathcal{A}_{\text{R-R}} \simeq
        V_{p+1}\ 2\pi(4\pi^2\ls^2)^{3-p}\ G_{9-p}(y)\,,
\end{equation}
donde $G_d(y) =
\tfrac{\pi^2}{4}\Gamma\left(\tfrac{d}{2}-1\right)\tfrac{1}{y^{d-2}}$
es la funci\' on de Green escalar en $d$ dimensiones.

Para obtener la tensi\'on y la carga de la D$p$-brana, podemos
comparar los resultados de~\eqref{pole} con c\'alculos de teor\ii as de
campos como la amplitud de intercambio de gravitones, dilatones y
campos de $R-R$ entre dos D-branas. Los dos ingredientes que
necesitamos son los propagadores y los acoplamientos. Los primeros se
obtienen de la acci\'on de supergravedad~\eqref{IIBE} y ~\eqref{IIAE} en
el Einstein frame, mientras que los \'ultimos de la acci\'on de volumen
de mundo. El resultado para los propagadores del gravit\'on $h_{\mu\nu}$
y del dilat\'on $\Phi$ con momento $k$ es 
\begin{equation}
	\langle h_{\mu\nu} h_{\rho\sigma} \rangle =
        -\frac{2i\kappa^2}{k^2}\left[\eta_{\mu\rho}\eta_{\nu\sigma}
          +\eta_{\mu\sigma}\eta_{\nu\rho} - \frac{1}{4}
          \eta_{\mu\nu}\eta_{\rho\sigma}\right]\,,\qquad \langle \Phi
        \Phi \rangle = - \frac{2i\kappa^2}{k^2}\,.
\end{equation}
Los dos diagramas de Feynman correspondientes al intercambio de
gravitones y dilatones suman la siguiente expresi\'on en el espacio de
configuraciones:
\begin{equation}
	\mathcal{A} = 2 V_{p+1}\ \tau_p^2 \kappa^2\ G_{9-p}(y)\,.
\end{equation}
La comparaci\'on con $\mathcal{A}_{\text{NS-NS}}$ da los siguientes
valores para $\tau_p$:
\begin{equation}\label{taup}
	\tau_p = \frac{\sqrt{\pi}(2\pi\ls)^{3-p}}{\kappa} =
        \frac{1}{(2\pi)^p \gs \ls^{p+1}}\,.
\end{equation}

Podemos realizar la misma comparaci\'on para el intercambio de campos
$C_{p+1}$ de $R-R$, con la normalizaci\'on usada en la acci\'on de
volumen de mundo~\eqref{wvE} obtenemos:
\begin{equation}\label{mup}
	\mu_p = \tau_p\,.
\end{equation}
Esto completa la determinaci\'on de la acci\'on de volumen de mundo,
ya que tenemos expresadas todas las cantidades en t\'erminos de las
cantidades de la teor\ii a de cuerdas $\gs$ y $\ls$.


==> intro.tex <==
% Title page and contents

\thispagestyle{empty}

\begin{flushright}
%{\small
%ITP-UU-03/67\\
%SPIN-03/43\\
%hep-th/0312070\\
%}
\end{flushright}

\begin{center}

\vspace{4cm}

{\Huge F\ii sica de $D$-branas en Teor\ii as de}\\

\vspace{0.5cm}

{\Huge Cuerdas No Cr\ii ticas}\\

\vspace{0.5cm}

%{\Huge Towards Realistic Gauge Theories}
%{\huge \protect\footnote{Based on the author's Ph.D. thesis ``Studies of the Gauge/String Theory Correspondence'', University of Torino, Italy, October 2003.}}

\vspace{1cm}

% Authors
{\Large Mauricio Bernardo Sturla}

\vspace{1cm}

% Institutions
{\large \emph{Facultad de Ciencias Exactas, Departamento de F\ii sica }}

\vspace{0.2cm}

{\large \emph{Universidad Nacional de La Plata }}

\vspace{0.4cm}

{\large \emph{Versi\'on Preliminar de Tesis de Doctorado }}

%{\large email: \verb|E.Imeroni@phys.uu.nl|}\\
\end{center}

%\vspace{2cm}


\newpage


\tableofcontents


==> introduction.tex <==
% "Introduction"

\chapter{Introduction}\label{c:introduction}

The physics of elementary particles, in the range of energies accessible to experiments, is described with very high precision by the Standard Model of particle physics. The Standard Model is a \emph{quantum gauge theory}, that is, a quantum field theory with local gauge symmetry.

This report deals with the study of quantum gauge theories in a somewhat  non-standard way, making use of different concepts and tools drawn from the fascinating arena of string theory, supersymmetry and gravity. This is what goes under the name of \emph{gauge/string theory} or \emph{gauge/gravity} correspondence.

It is a well known fact that string theory emerged as an attempt to explain strong interactions, and later evolved into a proposal for a theory able to incorporate all forces of nature into a coherent quantum framework. String theory has a lot of appealing properties for this role: just to give a brief list, it automatically includes gravity, does not present problems related to ultraviolet divergences, has no free adjustable parameters except for the scale, is a highly constrained and essentially unique theory, and includes many ideas which have been put forward in many attempts towards a unified description of nature, such as extra dimensions and supersymmetry. 

However, the interpretation of string theory as a putative ``theory of everything'' only makes the requirement of addressing gauge theories even stronger. In particular, if any sense for the description of the physical world should be given to string theory, it cannot avert from its ability to correctly describe the gauge theory interactions which are at the core of the Standard Model.

In fact, the possibility of using string theory as an efficient tool for computing gauge theory amplitudes has been known since the beginning of its history. A single diagram of perturbation theory of the open string reduces, in the field theory limit where the tension of the string is taken to infinity, to a sum of Feynman diagrams of a gauge theory, and this opens the way to many possible simplifications or alternative derivations of many gauge theory results.

During the last decade, the interplay between gauge theory and string theory has become even richer and fruitful. The discovery of \emph{Dirichlet branes}~\cite{Polchinski:1995mt}, or D-branes, that are new non-perturbative dynamical extended objects of diverse dimensions naturally present in type I and II string theories, has led to a new perspective on the way gauge theory is embedded in the superstring (besides of course making available a great tool to explore the landscape of connections between string theories via the exploitation of various perturbative and non-perturbative dualities).
%:Figure: Strings and branes
\begin{figure}
\begin{center}
\includegraphics[scale=.7]{dbranes}
\caption{{\small Strings and D-branes.}}
\label{f:dbranes}
\end{center}
\end{figure}

This new perspective on gauge theories from the string theory point of view has its central point in the \emph{double nature} of D-branes.
\begin{itemize}
\item On the one hand, D-branes admit a description in terms of perturbative \emph{open string theory}. They are defined as $p$-dimensional hyperplanes on which open string endpoints lie. The excitations of the open strings attached to a D-brane thus describe its dynamics. In particular, the massless states of the open string spectrum both represent the collective coordinates of a D-brane and give rise to a $(p+1)$-dimensional \emph{gauge theory} living on its world-volume.
\item On the other hand, D-branes can be regarded as sources of \emph{closed string} fields. They are non-perturbative \emph{classical solitons} of string theory, solutions of the low-energy supergravity equations of motion.
\end{itemize}
The deep consequences of the above complementarity of descriptions, which in some sense is a modern refinement of the older concept of \emph{open/closed string duality}, are the central theme of this report.

There is a particular example in which the twofold role of D-branes has proven extremely powerful for establishing a deep connection between gauge and string theory: it is the case of D3-branes in flat space, whose world-volume supports at low energies \Ne{4} superconformal Super Yang--Mills theory in four space-time dimensions.

A particular ``near-horizon'' limit of the geometry generated by the D3-branes has the surprising consequence of decoupling the bulk degrees of freedom from the ones living on the branes, while transforming the geometry into the product of five-dimensional Anti-de Sitter space times a five-sphere, where branes are replaced by Ramond-Ramond flux.

This is the basis of the Maldacena conjecture, or \emph{AdS/CFT duality}, which states that \emph{Type IIB string theory on \ads{} is dual to \Ne{4} Super Yang--Mills theory}~\cite{Maldacena:1998re,Gubser:1998bc,Witten:1998qj}. This is an exact duality, in the sense that the partition functions of the two theories are defined to be equivalent. This breakthrough achievement then relates two drastically different theories, a gauge theory and a gravitational theory, opening new perspectives on both of them, and is the deepest known example of gauge/gravity correspondence. The importance of this duality also resides in the fact that the strong coupling regime of the gauge theory has its dual closed string description in low-energy classical supergravity, thus allowing the opening of a computable window into non-perturbative gauge physics.

The AdS/CFT duality has been thoroughly tested in the recent years with great success. However, it is also worth pointing out one important limitation. The duality deals with \Ne{4} Super Yang--Mills theory, that is very far from providing a realistic description of the physical world. The main features which make \Ne{4} Super Yang--Mills theory ``unrealistic'' are:
\begin{itemize}
	\item it preserves a \emph{high amount of supersymmetry} (sixteen supercharges);
	\item it is a \emph{superconformal theory}.
\end{itemize}

Our interest here will be reporting on some attempts that have been pursued in order to generalize the correspondence beyond the above limitation. We will then study extensions of the gauge/string theory correspondence towards \emph{less supersymmetric and non-conformal gauge theories}. From what we said, it should be clear that this is a necessary step if we have in mind that ultimately the gauge/string correspondence should be able to give us relevant information on gauge theories which have something to do with the Standard Model which describes our physical world.

It is fair to say that, at the moment of writing, it has not yet proven possible to establish a full, exact duality between a gravitational and a gauge theory in the case in which the latter is non-conformal and preserves less than sixteen superysmmetries.

However, this does not mean that one cannot fruitfully use gravity to study these more ``realistic'' gauge theories. In fact, here we try giving a coherent, and reasonably self-contained, review of a particular approach to these extensions of the gauge/gravity correspondence. This approach is based on finding D-brane configurations in type II string theory that host on their world-volume some gauge theories of interest, and to study these theories by means of a dual gravitational description. There are some nice reviews of this and related approaches~\cite{Aharony:2002up,Bertolini:2003iv,Bigazzi:2003ui,DiVecchia:2003ne}, and of course more detailed references will be given in the following chapters.

How does one engineer configurations of D-branes supporting gauge theories with the requested properties? From what we said above, it should be clear that in order to pursue this program we have to act in two directions:
\begin{enumerate}
	\item \emph{Reduce supersymmetry}: the first step is to break part of the sixteen supercharges preserved by D-branes in flat space. This is achieved by appropriately choosing a \emph{closed string background} which breaks some amount of supersymmetry. For instance, one can consider type II strings on orbifolds or Calabi--Yau manifolds.
	\item \emph{Break conformal invariance}: in general, the theory living on a standard D-brane in such a background does not present any scale anomaly yet. In order to make it scale-anomalous, one has to act on the \emph{open string} side, by engineering configurations with particular properties, as for example D-brane having part of their world-volume wrapped on a non-trivial cycle of the ambient manifold.
\end{enumerate}
We will study in detail several D-brane setups in type II string theory, such as ``fractional'' D-branes on orbifolds and on the conifold and D-branes wrapped on supersymmetric cycles inside Calabi--Yau manifolds. The corresponding dual gauge theories are three- and four-dimensional scale-anomalous theories preserving eight or four supercharges. Among these, there are some gauge theories of more direct ``phenomenological'' interest, such as pure \Ne{1} and \Ne{2} Super Yang--Mills theory in four space-time dimensions.

Once a D-brane configuration yielding a gauge theory of interest has been constructed, the next step is finding the low-energy closed string description, in terms of a classical supergravity solution. We will see that the careful analysis of the solution yields interesting pieces of information on the dual gauge theory.  For example, depending on the context and the amount of unbroken supersymmetry, one can reproduce from classical supergravity relevant quantum gauge theory information such as:
\begin{itemize}
	\item \emph{at the perturbative level}: running gauge coupling constant, chiral anomaly, metric on the moduli space;
	\item \emph{at the non-perturbative level}: instanton action, gaugino condensation and chiral symmetry breaking, effective superpotential, tension of confining strings.
\end{itemize}
It is clear from the above list that the study of the generalizations of the gauge/string theory correspondence towards realistic gauge theories is an extremely rich subject, whose further study might very well lead to a deeper and better understanding of quantum gauge theories.

\subsection*{Organization of the paper}

This report is organized as follows. In chapter~\ref{c:dbranes}, after a brief summary of concepts and notations of perturbative string theory, we set the stage by introducing D-branes from different points of view. We introduce the perturbative notion of D-brane in open string theory, as a hypersurface where open strings end, and its interpretation as a solitonic solution of the low-energy closed string theory. This twofold nature of D-branes will be the central concept in all subsequent parts, and will be used to see how information on a gauge theory can be extracted from the classical geometry describing D-branes. This will be our first meeting with the gauge/gravity correspondence. Finally, concentrating on the case of D3-branes, we will consider the main example of the correspondence, by briefly introducing the duality between \Ne{4} Super Yang--Mills theory in four space-time dimensions and type IIB string theory compactified on  \ads.

Chapter~\ref{c:engineering} is devoted to the construction of brane configurations which allow obtaining on the world-volume of D-branes at low energies gauge theories with less than 16 supersymmetries and a running gauge coupling, namely, in the case of four-dimensional theories, broken conformal symmetry. The goal of these constructions is to get information on more ``realistic'' gauge theories. We will introduce some concepts about D-branes on non-trivial spaces, such as Calabi--Yau manifolds and orbifolds. In particular, we will extensively study, by means of simple examples, fractional D-branes on orbifolds and on the conifold, as well as D-branes wrapped on supersymmetric cycles. We will also establish some connections among these approaches, and between them and other approaches, such as stretched branes and ``geometric engineering''.

In chapter~\ref{c:8susy} we will present our first explicit constructions of gauge/gravity correspondence away from AdS/CFT. Two simple examples will be used to explain how one can obtain classical solutions corresponding to fractional D-branes on orbifolds and D-branes wrapped on a supersymmetric cycle inside a Calabi--Yau manifold, and extract from them information about the gauge theory living on the world-volume of the branes. The examples comprise a system of D4-branes wrapped on a two-cycle inside a Calabi--Yau twofold and a system of fractional D2/D6-branes on a \cz{} orbifold. In both cases, the dual gauge theory is scale-anomalous Super Yang--Mills theory in three space-time dimensions with 8 supercharges. After summarizing and generalizing the techniques derived with the aid of the examples, we apply them to two systems dual to \Ne{2} Super Yang--Mills theory in four space-time dimensions, namely a system of wrapped D5-branes and one of fractional D3/D7 branes.

Finally, chapter~\ref{c:4susy} reports on some attempts of constructing supergravity duals of \Ne{1} Super Yang--Mills theory in four dimensions, a theory with many qualitative similarities to non-supersymmetric QCD. In particular, we will see how relevant information can be extracted for the pure \Ne{1} theory from two classical solutions, one describing D5-branes wrapped on a two-cycle inside a Calabi--Yau threefold and one corresponding to fractional D-branes on the conifold. Finally, we will use another solution, corresponding to fractional D3-branes on a \czz{} orbifold, in order to study \Ne{1} SQCD with matter in the fundamental representation of the gauge group.

A final observation is that we will often use boxed ``inserts'', either in order to present material which is useful for the understanding, but not directly related to the logical development of the text, or to briefly sketch some topics when space does not allow more detailed explanations. As a first example, in insert~\ref{i:notations} on page~\pageref{i:notations} we summarize some of the notations and conventions we will be using throughout the paper.

%:Insert: Notations
\begin{Insert}{Notations}\label{i:notations}
We use the $(-\ +\ +\ \cdots\ +)$ signature of the metric, and set $\hbar=c=1$. We denote the string length as $\ls$ (the relation with the Regge slope is given by $\ls = \sqrt{\alpha'}$), and the closed string coupling as $\gs$.

When we write down space-time or world-volume actions, it is generally understood that the fields appearing in the action are \emph{fluctuations} around the vacuum expectation values of the fields. For instance, dilaton terms such as $e^{\Phi}$ do not contain the expectation value $\gs$.

We try to stick with the notation $X^\mu$ for coordinate fields in a world-sheet theory, and $x^\mu$ when referring generically to the coordinates of a space-time. However, especially when dealing with world-volume actions, some (usually non-confusing) mismatch of notation is unavoidable. In world-volume actions, we denote pull-backs of space-time fields with a hat.

We define the totally antisymmetric $\varepsilon$ symbols in $D$ dimensions as $\varepsilon^{012\dotsm (D-1)}=-\varepsilon_{012\dotsm (D-1)}=+1$. A differential $p$-form is defined as $\omega_p=\frac{1}{p!}\omega_{\mu_1 \dotsm\mu_p} dx^{\mu_1}\wedge\dotsm\wedge dx^{\mu_p}$, and its Hodge dual in $D$ dimensions is:
\begin{equation*}
	\hd{D}\omega_p=\frac{\sqrt{-\det G_D}}{p!(D-p)!} \varepsilon_{\nu_1\dotsm \nu_{D-p}\mu_1 		\dotsm\mu_p} \omega^{\mu_1\dotsm\mu_p}
		dx^{\nu_1}\wedge\dotsm\wedge dx^{\nu_{D-p}}\,.
\end{equation*}		
Moreover, $\hd{}$ denotes $\hd{10}$ and $\hde$ denotes $\hd{11}$. We will usually indicate the rank of a form with a subscript, as above, but we will often use just $B$ to denote the Neveu--Schwarz-Neveu--Schwarz two-form of string theory.

Finally, in order to describe configurations of D-branes, we often use diagrams as in the following example:
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
&0&1&2&3&4&5&6&7&8&9\\
\hline
D$4$ &$-$&$-$&$-$&$\bigcirc$&$\bigcirc$&$\cdot$&$\cdot$&$\cdot$&$\cdot$&$\cdot$\\
\hline
\end{tabular}
\begin{tabular}{cl}
$-$&denotes a direction \emph{longitudinal} to the world-volume\\
$\bigcirc$&denotes a \emph{compact} direction longitudinal to the world-volume\\
$\cdot$&denotes a direction \emph{transverse} to the world-volume\\
\end{tabular}
\end{center}
\end{Insert}
